The Efficacy of Transfer-based No-box Attacks on Image Watermarking: A Pragmatic Analysis

Watermarking approaches are widely used to identify if images being circulated are authentic or AI-generated. Determining the robustness of image watermarking methods in the ``no-box'' setting, where the attacker is assumed to have no knowledge about the watermarking model, is an interesting problem. Our main finding is that evading the no-box setting is challenging: the success of optimization-based transfer attacks (involving training surrogate models) proposed in prior work~\cite{hu2024transfer} depends on impractical assumptions, including (i) aligning the architecture and training configurations of both the victim and attacker's surrogate watermarking models, as well as (ii) a large number of surrogate models with potentially large computational requirements. Relaxing these assumptions i.e., moving to a more pragmatic threat model results in a failed attack, with an evasion rate at most $21.1\%$. We show that when the configuration is mostly aligned, a simple non-optimization attack we propose, OFT, with one single surrogate model can already exceed the success of optimization-based efforts. Under the same $\ell_\infty$ norm perturbation budget of $0.25$, prior work~\citet{hu2024transfer} is comparable to or worse than OFT in $11$ out of $12$ configurations and has a limited advantage on the remaining one. The code used for all our experiments is available at \url{https://github.com/Ardor-Wu/transfer}.

==> contents/notes.tex <==
\section{Notes}

We study the robustness of image watermarking. 
\subsection{Research Gap}
We studied two papers on this topic:

\begin{enumerate}
    \item \textbf{\citet{jiang2023evading}:} \textcolor{red}{could you add some notes on what the method is?}
    \begin{enumerate}
        \item (General) The setting is too easy for the attacker.
        \item The white-box scenario is impractical. Method: WEvade-W-II, we do not care white box
        \item Black box
        \begin{enumerate}
            \item WEvade-B-S: surrogate encoder to convert to  white box, not a good method
            \item WEvade-B-Q still needs to query the detector.
            
            WEvade-B-Q=HopSkipJump+JPEG initialization + early stopping by checking perturbation
            
            HopSkipJump = random initialization + walking towards $I_w$ while guarantee evasion + stop until query budget used up 


        \end{enumerate}
    \end{enumerate}
    
    \item \textbf{\citet{saberi2023robustness}:} \textcolor{red}{could you add some notes on what the method is?}
    \begin{enumerate}
        \item \textbf{Low perturbation:} Low perturbation methods include \texttt{watermarkDM}, \texttt{RivaGAN}. Diffusion purification \citet{nie2022diffusion} can attack them, by adding the Gaussian noise and then remove with denoising diffusion models.
        \item \textbf{High perturbation:} Train substitute and Projected Gradient Descent (PGD), which is black-box, yet more complex than what we are trying.
        \item \textbf{Spoofing:} We do not care about their spoofing defined as such making false positives.
        \item \textbf{Used as codebase:} We start from their implementation.
    \end{enumerate}
\end{enumerate}
\subsubsection{Target Watermarking Methods}

\begin{enumerate}
    \item \textbf{hidden \citep{zhu2018hidden}:} The basic encoder-decoder watermarking.
    \item \textbf{MBRS \citep{jia2021mbrs}:} Hidden with JPEG robustness added using Mini-Batch of Real and Simulated JPEG Compression.
    \item \textbf{stegaStamp \citep{tancik2020stegastamp}:} Encoder-decoder with added corruption robustness, using the data collected with printing, re-imaging, and other augmentations.
    \item \textbf{watermarkDM \citep{zhao2023recipe}:} watermark is added to the training data using a convolutional network. Then the training data is fed to a Diffusion Model (DM) for training - nothing specific to DM.
    \item \textbf{rivaGan \citep{zhang2019robust}:} Using attention-based structure instead of CNN.

\end{enumerate}


\textcolor{red}{what are some other related works? in the figures below, you have multiple attacks? need a line each about each of them?}

\subsection{Our attack idea}
Our spoofing attack:
Train another watermark attack (evading watermark detection by adding another watermark to interfere with the previous one)

Image $I$ + watermark $A$ with secret message $S_A$ + watermark $B$ with secret message $S_B$: Can $S_A$ still be detected? \textcolor{red}{or can $S_B$ also be detected?} Not explored, yet $S_B$ should be detected as $I$ with watermark $S_A$ is still an valid image. 

\subsection{Direct Transfer}

We tried a direct transfer using by truncating the secret message \textcolor{red}{what does truncating mean?} when necessary. More specifically, we use the checkpoints and only check the first 30 bits as the shortest secret only has 30 bits; for the remaining part, we set it to all 0 when applying. It is not successful, as it works iff the same encoder. \textcolor{red}{could you please clarify this statement?} \textcolor{red}{also, what is random + bitflip?} The attack is to add a second watermark to the watermarked images. We use the official checkpoints. So, for diagonal, a second watermark is added using the same encoder. "Random" means that the second watermark's secret is random. "Bitflip" means the second watermark's secret is a bitwise flip from the first one. Removed \texttt{dwtDct} and \texttt{dwtDctSvd} as they are not learning-based methods. Only diagonal points have significantly reduced the AUROC values, meaning these are the only working ones.

\begin{figure}[H]
\begin{center}
\includegraphics[width=4.0in]{figures/DirectRandomUpdated.png} % Include the image file
\end{center}
\caption{Random}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=4.0in]{figures/DirectFlipUpdated.png} % Include the image file
\end{center}
\caption{Bitflip}
\end{figure}

\subsection{Rethink}

\subsubsection{Different Configs}

\textbf{Dataset, architecture, secret length}

Details can be found here: \url{https://docs.google.com/spreadsheets/d/1_zZZU4tQTNj0_H4ejPBrk0VIxydqa5XvVZzS97UMxrU/edit?gid=0#gid=0}

Noise/augmentations added are also important yet not fully explored.



\textcolor{red}{what is $h$?}

\textbf{Step 4:} Decode the modified latent, i.e., $x' = \text{Dec}(e')$.

Consider this process, we scope the limit to \texttt{MBRS} \citep{jia2021mbrs}, StegaStamp \citep{tancik2020stegastamp}, watermarkDM \citep{zhao2023recipe}, rivaGAN \citep{zhang2019robust} (and later added \textsc{Hidden} \citep{zhu2018hidden}).



Considering the similarity, we focus on \texttt{MBRS} and \textsc{Hidden} as a pair first.

\subsection{Alignment Case Study: \texttt{MBRS} and \textsc{Hidden}}
\subsubsection{Clustering}
Clustering shows that \texttt{MBRS} and \textsc{Hidden} features $e$ and $h$, defined as above, \textcolor{red}{what does feature mean? based on the notation in section 1.4?} are well separated before retraining. For $g$, the visualization is degenerated. No valid results after retraining. \textcolor{red}{what does this mean?} The visualization we made was before convergence. \textcolor{red}{what happened after convergence? } We did not do feature clustering after completely aligning at the end of last semester.

\begin{figure}[H]
\begin{center}
\includegraphics[width=4.0in]{figures/Clustering1.png} 
\end{center}
\caption{TSNE for e}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=4.0in]{figures/Clustering2.png} 
\end{center}
\caption{TSNE for h}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=4.0in]{figures/e-link.png} 
\end{center}
\caption{No significant pattern when we link the features $e$ for the same image}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=4.0in]{figures/h-link.png} 
\end{center}
\caption{No significant pattern when we link the features $h$ for the same image}
\end{figure}

\subsection{Retraining}
\subsubsection{Aligned configs}

\begin{itemize}
    \item \textbf{Methods:} \texttt{MBRS} and \textsc{Hidden}, both retrained
    \begin{itemize}
        \item \textbf{Learning rate:} $1 \times 10^{-3}$
        \item \textbf{Dataset:} \textsc{Hidden} (COCO train + COCO val)
        \item \textbf{Number of samples:} 10,000 (train) + 1,000 (val)
        \item \textbf{Secret message length (m):} 36
        \item Removed noise added during training, though JPEG noise added in MBRS is their main contribution.
    \end{itemize}
\end{itemize}

\subsubsection{Results}
The attack was not successful. Watch for the highlighted boxes for transfer between \texttt{MBRS} and \textsc{Hidden} and WatermarkDM attacking these two.

\begin{figure}[H]
\begin{center}
\includegraphics[width=3.0in]{figures/Results2.png} 
\end{center}
\caption{Random}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=3.0in]{figures/Results1.png} 
\end{center}
\caption{Bitflip}
\end{figure}

\subsubsection{Ablation}

We trained \texttt{Hidden} with $2000$ epochs and a smaller learning rate $10^{-4}$ with all other configs the same as described above. We confirmed that a large $m$ causes the previous attempt to retrain \textsc{Hidden} to align with \texttt{MBRS} to fail.

\begin{figure}[H]
\begin{center}
\includegraphics[width=3.0in]{figures/ablationRandom.png} 
\end{center}
\caption{Random}
\end{figure}

\begin{figure}[H]
\begin{center}
\includegraphics[width=3.0in]{figures/ablationFlip.png} 
\end{center}
\caption{Bitflip}
\end{figure}
\subsection{Previous Storyline}

We are at step 5 (or 6 is no longer useful):

\begin{enumerate}[label=Step \arabic*:]
    \item There are attacks on image watermarking. For example, Neil Gong’s attacks.
    \item A possible spoofing attack is simpler (and more black-box).
    \item Naive spoofing attack fails - why?
    \item Different watermarking strategies have different configurations, e.g., secret message length, training data, architecture, etc.
    \item When we fix the configuration, is it more effective? - No by far.
    \item Why? What if the dataset is not the same but similar (e.g., IMO, ImageNet vs ImageNetV2)? \textcolor{red}{does this mean that we have not fixed the dataset during our experiments?} We chose the most similar pair, \texttt{MBRS} and \texttt{HIDDEN} and fixed the dataset to be the same. For others, not yet, but now we can expect a similar dataset will not work, given the same dataset is not working.
    \item Attack effectiveness when secret length varies (can be parallel to step 6).
\end{enumerate}

\subsection{Non-optimization Attack Algorithm}

\textbf{Notations}

\begin{itemize}
    \item Let \( k \) be the number of surrogate models.
    \item For \( i = 1, \dotsc, k \):
    \begin{itemize}
        \item \( E_i(x, s) \) is the encoder of the \( i \)-th surrogate model, which embeds secret \( s \) into image \( x \), producing a watermarked image.
        \item \( d_i(x) \) is the decoder of the \( i \)-th surrogate model, extracting the secret from image \( x \).
    \end{itemize}
    \item \( r \) is the attack budget (maximum allowable perturbation norm).
    \item \( \text{aggr} \) is an aggregation function (e.g., element-wise mean or median) used to combine the perturbations.
\end{itemize}

\textbf{Input}

\begin{itemize}
    \item Watermarked image from the target model: \( x' \).
    \item Surrogate models: \( \{E_i(x, s),\ d_i(x)\}_{i=1}^k \).
\end{itemize}

\textbf{Output}

\begin{itemize}
    \item Attacked watermarked image: \( x_{\text{attk}} \).
\end{itemize}

\textbf{Algorithm}

\begin{enumerate} \item \textbf{Compute Individual Perturbations}

For each surrogate model \( i = 1, \dotsc, k \), calculate:

\[
\varepsilon_i = E_i\left(x',\, \overline{d_i(x')}\,\right) - x',
\]

where \( \overline{d_i(x')} \) denotes the bitwise complement (flip) of the decoded secret \( d_i(x') \).

\item \textbf{Aggregate Perturbations}

Combine the individual perturbations using the aggregation function \( \text{aggr} \):

\[
\varepsilon = \text{aggr}\left(\varepsilon_1,\, \varepsilon_2,\, \dotsc,\, \varepsilon_k\right).
\]

The aggregation function \( \text{aggr} \) can be the pixel-wise mean or median.

\item \textbf{Normalize Perturbation (if necessary)}

If normalization is required to adhere to the attack budget $\|\varepsilon\|_{\infty} \leq r$
 norm, adjust \( \varepsilon \) by clamping its values so that each element lies within \(-r\) and \( r \):

\[
\varepsilon_i = \begin{cases}
    -r, & \text{if } \varepsilon_i < -r, \\
    \varepsilon_i, & \text{if } -r \leq \varepsilon_i \leq r, \\
    r, & \text{if } \varepsilon_i > r.
\end{cases}
\]

This ensures that the perturbation's individual components do not exceed the attack budget \( r \) in magnitude.

\item \textbf{Generate Attacked Image}

Apply the aggregated perturbation to the original watermarked image:

\[
x_{\text{attk}} = x' + \varepsilon.
\]
\end{enumerate}
\textbf{Summary}

This algorithm generates an attacked image \( x_{\text{attk}} \) by computing perturbations that flip the decoded secrets of surrogate models, aggregating these perturbations using \( \text{aggr} \), normalizing them to respect the attack budget in the \( \ell_\infty \)-norm, and applying the result to the original watermarked image.



==> figures/RT_table.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|c|}
\hline
\textbf{Methods} & \textbf{Time (s)} \\
\hline
\citet{hu2024transfer} & 2493.0594\\
\hline
\citet{saberi2023robustness} Diffpure - 0.05 & 69.7701 \\
\citet{saberi2023robustness} Diffpure - 0.1 & 138.3874 \\
\citet{saberi2023robustness} Diffpure - 0.2 & 274.6078 \\
\citet{saberi2023robustness} Diffpure - 0.3 & 411.7274 \\
\hline
Ours - unnormalized & \textbf{0.3853} \\
Ours - normalized & \textbf{0.3987} \\
\hline
\end{tabular}
\caption{Comparison of Running Times}
\label{RT}
\end{table}


==> figures/quality_table.tex <==
\begin{table*}[h!]
\centering
\tiny
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{Methods} & \textbf{\# Matched Bits} & \textbf{Watermarked?} & \textbf{LPIPS} & \textbf{$l_\infty$} & \textbf{Overall Bit-wise Acc.} & \textbf{Evasion Rate} & \textbf{Overall LPIPS} & \textbf{Overall $l_\infty$} \\
\hline

Unattacked & 29 & \ding{51} & / & / & / & 0.005 & / & /\\
\hline

\citet{hu2024transfer} & 12 & \ding{55} &  0.0042895 &  0.25 & 0.4702  &  0.998 &  0.0177 &  0.1951 \\
\hline
DP 0.05 \citep{saberi2023robustness} & 26 & \ding{51} & 0.0506 & 0.4961 & 0.8078 & 0.690 & 0.0797 & 0.3410\\
DP 0.1 \citep{saberi2023robustness} & 22 & \ding{55} & 0.0591 & 0.5662 & 0.6802 & 0.974 & 0.1242 & 0.4482 \\
DP 0.2 \citep{saberi2023robustness} & 16 & \ding{55} & 0.0817 & 0.6707 & 0.5685 & 1.000 & 0.1623 & 0.6155 \\
DP 0.3 \citep{saberi2023robustness} & 16 & \ding{55} & 0.1087 & 0.8732 & 0.5299 & 1.000 & 0.1921 & 0.7966 \\
\hline
Ours - Unnorm & 17 & \ding{55} & 0.0763 & 0.4954 & 0.4907 & 1.000 & 0.0781 & 0.4682\\
Ours - Clamp & 21 & \ding{55} & 0.0709 & 0.2500 & 0.4974 & 1.000 & 0.0767 & 0.2488\\
\hline
\end{tabular}
\caption{Comparison of Performance Metrics}
\label{Metrics}
\end{table*}


==> style/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


